Improving robustness against common corruptions by covariate shift adaptation

Today's state-of-the-art machine vision models are vulnerable to image corruptions like blurring or compression artefacts, limiting their performance in many real-world applications. We here argue that popular benchmarks to measure model robustness against common corruptions (like ImageNet-C) underestimate model robustness in many (but not all) application scenarios. The key insight is that in many scenarios, multiple unlabeled examples of the corruptions are available and can be used for unsupervised online adaptation. Replacing the activation statistics estimated by batch normalization on the training set with the statistics of the corrupted images consistently improves the robustness across 25 different popular computer vision models. Using the corrected statistics, ResNet-50 reaches 62.2% mCE on ImageNet-C compared to 76.7% without adaptation. With the more robust DeepAugment+AugMix model, we improve the state of the art achieved by a ResNet50 model up to date from 53.6% mCE to 45.4% mCE. Even adapting to a single sample improves robustness for the ResNet-50 and AugMix models, and 32 samples are sufficient to improve the current state of the art for a ResNet-50 architecture. We argue that results with adapted statistics should be included whenever reporting scores in corruption benchmarks and other out-of-distribution generalization settings.

==> figs/02-method/model-new.tex <==
\definecolor{bb}{HTML}{b3cde3}
\definecolor{gg}{HTML}{ccebc5}
\definecolor{or}{HTML}{fbb4ae}
\definecolor{lila}{RGB}{141,160,203}

\begin{figure}
\begin{center}

\tikzset{axarrow/.style={-latex,draw=black!40,thick}}
\tikzset{elarrow/.style={-latex,draw=black,thick}}

\newcommand{\drawax}{
    \draw[axarrow] (-2,0) to (2,0);
    \draw[axarrow] (0, -2) to (0,2);
    \draw[dashed] (-2,-2) to (2,2);
}

\begin{tikzpicture}[scale=.6]
\tikzmath{%
%target statistics
\mutx = .5; \muty = -1.;
\anglet = -45;
\utx = cos(\anglet); \uty = sin(\anglet);
\vtx = cos(\anglet+90); \vty =  sin(\anglet+90);
\uut = 4; \vvt = 2; % eigenvalues
\squut = sqrt(\uut); \sqvvt = sqrt(\vvt); % eigenvalues
%source statistics
\musx = 1.5; \musy = 2.;
\angles = 45;
\usx = cos(\angles); \usy = sin(\angles);
\vsx = cos(\angles+90); \vsy =  sin(\angles+90);
\uus = 5; \vvs = 1; % eigenvalues
\squus = sqrt(\uus); \sqvvs = sqrt(\vvs);
%target normalized with source statistics
\usmuts = \usx*(\mutx - \musx) + \usy*(\muty - \musy);
\vsmuts = \vsx*(\mutx - \musx) + \vsy*(\muty - \musy);
\mutsx = \usmuts*\usx/\squus + \vsmuts*\vsx/\sqvvs; %new mean 
\mutsy =  \usmuts*\usy/\squus + \vsmuts*\vsy/\sqvvs; %new mean
\anglets = \anglet - \angles;
\uuts = 1.5*\uut/\uus;
\vvts = 1.5*\vvt/\vvs;
%source normalized with target statistics
\usmust = \utx*(\musx - \mutx) + \uty*(\musy - \muty);
\vsmust = \vtx*(\musx - \mutx) + \vty*(\musy - \muty);
\mustx = \usmust*\utx/\squut + \vsmust*\vtx/\sqvvt; %new mean 
\musty =  \usmust*\uty/\squut + \vsmust*\vty/\sqvvt; %new mean
\anglest = \angles - \anglet;
\uust = 1.5*\uus/\uut;
\vvst = 1.5*\vvs/\vvt;
}
%\tikzmath{%
%\covtxx = \uu * \ux * \ux + \vv * \vx * \vx;
%\covtyy = \uu * \uy * \uy + \vv * \vy * \vy;
%\covtxy = \uu * \ux * \uy + \vv * \vx * \vy;
% inverse matrix
%\icovtxx = (1.0)/\uu * \ux * \ux + (1.0)/\vv * \vx * \vx;
%\icovtyy = (1.0)/\uu * \uy * \uy + (1.0)/\vv * \vy * \vy;
%\icovtxy = (1.0)/\uu * \ux * \uy + (1.0)/\vv * \vx * \vy;
%}

\begin{scope}[shift ={(-1,0)}] 
%source ellipse

    %\node[above right] at (\musx - \usx - 1.5, \musy + 1.5) {source/train};
    \node[below right] at (\musx - \usx-1.5, \muty - \vty - 2.2) {unnormalized feature spaces};
    
    \fill[rotate around = {\angles:(\musx, \musy)}, lila] (\musx,\musy) ellipse ({\squus} and \sqvvs);
    
    \fill[or, rotate around={\angles:({0.5*(2*\musx + \sqvvs*\vsx)}, {0.5*(2*\musy +\sqvvs*\vsy)})}] ({0.5*(2*\musx + \sqvvs*\vsx)}, {0.5*(2*\musy +\sqvvs*\vsy)}) ellipse ({0.6*\squus} and {0.35*\sqvvs});
    \fill[gg, rotate around={\angles:({0.5*(2*\musx - \sqvvs*\vsx)}, {0.5*(2*\musy -\sqvvs*\vsy)})}] ({0.5*(2*\musx - \sqvvs*\vsx)}, {0.5*(2*\musy -\sqvvs*\vsy)}) ellipse ({0.6*\squus} and {0.35*\sqvvs});
    
    \draw[elarrow] (\musx, \musy) to (\musx + \squus*\usx, \musy + \squus*\usy);
    \draw[elarrow] (\musx, \musy) to (\musx + \sqvvs*\vsx, \musy + \sqvvs*\vsy);
    
    %target ellipse
    %\node[above right] at (\musx - \usx - 1.5, \muty + 0.2) {target/test};
    %\node[above right] at (\musx - \usx - 1.5, \muty - 0.25) {(non-i.i.d.)};
    
    \draw[axarrow] (\musx + 2, \musy + 1.6) to node[above] {source domain} (\mutx + 5.5, \musy + 1.6);
    \draw[axarrow] (\musx + 2, \muty + 0.3) to node[above] {target domain} (\mutx + 5.5, \muty + 0.3);
    
    \fill[lila,rotate around = {\anglet:(\mutx, \muty)}] (\mutx,\muty) ellipse ({\squut} and \sqvvt);
    
    \fill[or,rotate around={\anglet:({0.5*(2*\mutx - \squut*\utx)}, {0.5*(2*\muty -\squut*\uty)})}] ({0.5*(2*\mutx - \squut*\utx)}, {0.5*(2*\muty - \squut*\uty)}) ellipse ({0.3*\squut} and {0.7*\sqvvt});
    \fill[gg,rotate around={\anglet:({0.5*(2*\mutx + \squut*\utx)}, {0.5*(2*\muty + \squut*\uty)})}] ({0.5*(2*\mutx + \squut*\utx)}, {0.5*(2*\muty +  \squut*\uty)}) ellipse ({0.3*\squut} and {0.7*\sqvvt});
    
    \draw[elarrow] (\mutx, \muty) to (\mutx - \squut*\utx, \muty - \squut*\uty);
    \draw[elarrow] (\mutx, \muty) to (\mutx + \sqvvt*\vtx, \muty + \sqvvt*\vty);
    
    \draw[axarrow] (\musx - \usx - 1.5, \muty - \vty - 1.5) to (\mutx + \vtx + 1.5, \muty - \vty - 1.5);
    \draw[axarrow] (\musx - \usx - 1.5, \muty - \vty - 1.5) to (\musx - \usx - 1.5, \musy+ \vsy + 1.5);

\end{scope}

\begin{scope}[shift ={(\mutx + \vtx + 6, \musy+ \vsy )}] 

    \fill[lila] (0,0) circle (1.5cm);
    \fill[or] ({\angles + 90}:0.75cm) circle ({0.3*1.5cm});
    \fill[gg] ({\angles - 90}:0.75cm) circle ({0.3*1.5cm});
    
    \drawax
    \draw[elarrow] (0,0) to (\angles:1.5cm);
    \draw[elarrow] (0,0) to ({\angles + 90}:1.5cm);

\end{scope}

\begin{scope}[shift ={(\mutx + \vtx + 6, \muty - \vty)}] 

    \fill[lila, rotate around = {\anglets:(0.2*\mutsx, 0.2*\mutsy)}] ({0.2*\mutsx},{0.2*\mutsy}) ellipse ({sqrt(\uuts)} and {sqrt(\vvts)});
    
    \fill[or,rotate around = {\anglets:({0.5*(0.4*\mutsx - cos(\anglets)*sqrt(\uuts))},{0.5*(0.4*\mutsy - sin(\anglets)*sqrt(\uuts))})}] ({0.5*(0.4*\mutsx - cos(\anglets)*sqrt(\uuts))},{0.5*(0.4*\mutsy - sin(\anglets)*sqrt(\uuts))}) ellipse ({0.3*sqrt(\uuts)} and {0.7*sqrt(\vvts)});
    
    \fill[gg, rotate around = {\anglets:({0.5*(0.4*\mutsx - cos(\anglets-180)*sqrt(\uuts))},{0.5*(0.4*\mutsy - sin(\anglets-180)*sqrt(\uuts))})}] ({0.5*(0.4*\mutsx - cos(\anglets-180)*sqrt(\uuts))},{0.5*(0.4*\mutsy - sin(\anglets-180)*sqrt(\uuts))}) ellipse ({0.3*sqrt(\uuts)} and {0.7*sqrt(\vvts)});
    
    \drawax

    
    \draw[elarrow] ({0.2*\mutsx},{0.2*\mutsy}) to ({0.2*\mutsx - cos(\anglets)*sqrt(\uuts)},{0.2*\mutsy - sin(\anglets)*sqrt(\uuts)});
    \draw[elarrow] ({0.2*\mutsx},{0.2*\mutsy}) to ({0.2*\mutsx - cos(\anglets-90)*sqrt(\vvts)},{0.2*\mutsy - sin(\anglets-90)*sqrt(\vvts)});
    
    
    \node[below right] at (-2, -2.2) {norm w/source};

\end{scope}

\begin{scope}[shift ={(\mutx + \vtx + 10.5, \musy+ \vsy )}] 

    \fill[lila, rotate around = {\anglest:(0.2*\mustx, 0.2*\musty)}] ({0.2*\mustx},{0.2*\musty}) ellipse ({sqrt(\uust)} and {sqrt(\vvst)});
    
    \fill[or, rotate around = {\anglest:({0.5*(0.4*\mustx - cos(\anglest)*sqrt(\uust))},{0.5*(0.4*\musty - sin(\anglest)*sqrt(\uust))})}] ({0.5*(0.4*\mustx - cos(\anglest)*sqrt(\uust))},{0.5*(0.4*\musty - sin(\anglest)*sqrt(\uust))}) ellipse ({0.3*sqrt(\uust)} and {0.7*sqrt(\vvst)});
    
    \fill[gg, rotate around = {\anglest:({0.5*(0.4*\mustx - cos(\anglest-180)*sqrt(\uust))},{0.5*(0.4*\musty - sin(\anglest-180)*sqrt(\uust))})}] ({0.5*(0.4*\mustx - cos(\anglest-180)*sqrt(\uust))},{0.5*(0.4*\musty - sin(\anglest-180)*sqrt(\uust))}) ellipse ({0.3*sqrt(\uust)} and {0.7*sqrt(\vvst)});
    
    \drawax
    
    \draw[elarrow] ({0.2*\mustx},{0.2*\musty}) to ({0.2*\mustx - cos(\anglest-180)*sqrt(\uust)},{0.2*\musty - sin(\anglest-180)*sqrt(\uust)});
    \draw[elarrow] ({0.2*\mustx},{0.2*\musty}) to ({0.2*\mustx - cos(\anglest-90)*sqrt(\vvst)},{0.2*\musty - sin(\anglest-90)*sqrt(\vvst)});

\end{scope}

\begin{scope}[shift ={(\mutx + \vtx + 10.5, \muty - \vty)}] 

    \fill[lila] (0,0) circle (1.5cm);
    \fill[or] ({\anglet - 180}:0.75cm) circle ({0.3*1.5cm});
    \fill[gg] ({\anglet}:0.75cm) circle ({0.3*1.5cm});
    
    \drawax
    \draw[elarrow] (0,0) to ({\anglet - 180}:1.5cm);
    \draw[elarrow] (0,0) to ({\anglet + 90}:1.5cm);
    
    \node[below right] at (-2, -2.2) {norm w/target};

\end{scope}

\end{tikzpicture}
\end{center}
\caption{%
\todo{caption}
}
\end{figure}

==> figs/02-method/model.tex <==
\begin{figure}[tp]
    \centering
   %\resizebox{0.9\textwidth}{!}{\input{figs/02-method/model.pdf_tex}}
   \includegraphics[width=0.9\textwidth]{figs/02-method/Fig1_texfont.pdf}
    \caption{%
    We assume that a large fraction of domain shift between the train (source) distribution and the test (target) distribution can be attributed to changes in feature-wise mean and variance in intermediate network layers (A).
    In this view, normalizing with train statistics (B) yields a decision boundary (B, upper) not compatible with target features normalized with the wrong statistics (B, lower).
    Instead, our scheme proposes to re-compute the %correct
    statistics on the test dataset and employ these for normalization (C, lower).
    }
    \label{fig:model}
\end{figure}

==> figs/04-results/ablation-priors.tex <==
\pgfplotsset{every tick label/.append style={font=\footnotesize}}
\pgfmathsetlengthmacro\MajorTickLength{
  \pgfkeysvalueof{/pgfplots/major tick length} * 4
}

\pgfkeys{/pgfplots/priorplot/.style={
    width=0.4\textwidth,
    height=0.4\textwidth,
    cycle list/RdPu-9,
    xlabel=Batch size,
    ylabel={mCE},
    xtick=      {1,2,4,8,16,32,64,128,256,512,1024,2048,4096},
    xticklabels={1, , ,8,  ,  ,64,   ,   ,512,    ,    ,4096},
    xmin=1,
    xmax=4096,
    ymin=40,
    ymax=100,
    legend pos=north east,
    legend columns=5,
    transpose legend,
    legend style={draw = none, at={(1.2,0.99), font=\tiny}, name=legend},
    legend image post style={line width = 3pt}
}}

\begin{figure}[htp]
\begin{center}
\begin{tikzpicture}
\begin{axis}[tuftelike,priorplot,xmode=log,title=ResNet50]

\addplot+ [mark=none, draw = gray] table [x=batchsize, y=0.0]{data/batchsize/priors-rn50.tsv};
\foreach \ccol in {1.0, 2.0, 4.0, 8.0, 16.0, 64.0, 256.0, 1024.0}{
    \addplot+ [mark=none] table [x=batchsize, y=\ccol]{data/batchsize/priors-rn50.tsv};
}
\addplot+ [gray, mark=none, dashed] table [x=batchsize, y=infty]{data/batchsize/priors-rn50.tsv};

\end{axis}
\begin{axis}[tuftelike,priorplot,xmode=log,at={(.5\textwidth,0)},title=Augmix]

\addplot+ [mark=none, draw = gray] table [x=batchsize, y=0.0]{data/batchsize/priors-am.tsv};
\addlegendentry{$N=0$}
%\pgfplotsset{cycle list shift=-1}


\foreach \ccol in {1.0, 2.0, 3.0, 4.0, 5.0, 6.0, 7.0, 8.0, 16.0, 64.0, 256.0, 1024.0}{
    \addplot+ [mark=none] table [x=batchsize, y=\ccol]{data/batchsize/priors-am.tsv};
    \addlegendentryexpanded{$N=\ccol$}
}
\addplot+ [gray, mark=none, dashed] table [x=batchsize, y=infty]{data/batchsize/priors-am.tsv};
\addlegendentry{$N=\infty$}

\end{axis}
\end{tikzpicture}
\end{center}
\end{figure}

==> figs/04-results/imagenet-r.tex <==
\newcommand{\insrulesINR}{%
        \cmidrule( r){1-1}
        \cmidrule(lr){2-3}
}

\begin{table}[!h]
\centering
\tiny\sffamily
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\begin{tabularx}{\textwidth}{@{}l@{}l@{}X}
\begin{tabular}[t]{lrr}
\multicolumn{3}{l}{%
T1: ImageNet-R (n=2048), top-1 error.
}
\\
\toprule
Model, adaptation: & base & adapt \\
\insrulesINR
ResNet50                   &  63.8 &   59.9 \\
Fixup                      &  61.2 &    --- \\
GroupNorm                  &  65.0 &    --- \\
\insrulesINR
SIN                        &  58.6 &   54.2 \\
ANT                        &  61.0 &   58.0 \\
ANT+SIN                    &  53.8 &   52.0 \\
AugMix (AM)                &  59.0 &   55.8 \\
DeepAug (DAug)              &  57.8 &   52.5 \\
DAug + AM           &  53.2 &   48.9 \\
\insrulesINR
DAug + AM (RNXt101) &  \textbf{47.9} &   \textbf{44.0} \\
\bottomrule
\end{tabular}
&
\begin{tabular}[t]{l}
\begin{tabular}[t]{lrr}
\multicolumn{3}{l}{%
Table 2: New models on IN-C (n=2048), mCE
}\\
\toprule
Model                      &  base  & adapt  \\
\midrule
DeepAug            &  60.36 &  49.44 \\
DeepAug+AugMix     &  53.55 &  45.36 \\
\midrule
DeepAug+AugMix+RNXt101 &  \textbf{44.52} &  \textbf{37.96} \\
\bottomrule
\end{tabular}\\
\\
\begin{tabular}{lcc}
\multicolumn{3}{c}{T.\,3a: ObjectNet evaluation (n = 512), acc}\\
\toprule
ResNet50 model & top-1 & top-5 \\
\midrule
BatchNorm w/o adapt & 21.85 & 39.09 \\
BatchNorm w/ adapt & 24.04 & 41.15 \\
GroupNorm & \textbf{29.18} & \textbf{50.24} \\
Fixup & 28.52 & 48.56 \\
\bottomrule
\end{tabular}
\begin{tabular}{cc}
\multicolumn{2}{c}{T.\,3b: Mixed IN-C, err}\\
\toprule
top-1 & top-5 \\
\midrule
61.08 &  40.81 \\
60.87 &  40.31 \\
57.25 &  35.97 \\
\textbf{56.83} &  \textbf{35.43} \\
\bottomrule
\end{tabular}
\end{tabular}
\end{tabularx}
\end{table}

==> figs/05-analysis/imagenet-r.tex <==
\newcommand{\insrulesINRTable}{%
        \cmidrule( r){1-1}
        \cmidrule(lr){2-4}
}

\begin{table}[tpb]\footnotesize
    \begin{minipage}{.5\linewidth}
      \centering
    \small
    \captionsetup{width=.75\textwidth}
    \caption{%
Adaptation improves the performance of robustified models on IN-R. We consider $n=2048$ for adaptation.
    }
\scriptsize
\begin{tabular}[t]{lrcr}
\multicolumn{3}{l}{%
ImageNet-R (n=2048), top-1 error.
}
\\
\toprule
Model, adaptation: & base & adapt & $\Delta$ \\
\insrulesINRTable
ResNet50                   &  63.8 &   59.9 & -3.9 \\
Fixup                      &  61.2 &    --- & --- \\
GroupNorm                  &  65.0 &    ---  & ---\\
\insrulesINRTable
SIN                        &  58.6 &   54.2 & -4.4 \\
ANT                        &  61.0 &   58.0 & -3.0 \\
ANT+SIN                    &  53.8 &   52.0 & -1.8 \\
AugMix (AM)                &  59.0 &   55.8 & -3.2 \\
DeepAug (DAug)              &  57.8 &   52.5 & -5.3\\
DAug + AM           &  53.2 &   48.9 & -4.3 \\
\insrulesINRTable
DAug + AM (RNXt101) &  \textbf{47.9} &   \textbf{44.0} & -3.9\\
\bottomrule
\end{tabular}
    \label{tbl:imagenet-r}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
    \small
    \captionsetup{width=.75\textwidth}
    \captionof{figure}{Top-1 error on ImageNet-R as obtained by a vanilla model w/ and w/o adaptation compared to the AugMix and DeepAug+AugMix models w/o adaptation.}
    %\caption{%
%
%    }
     \includegraphics[width=0.9\textwidth]{figs/05-analysis/inr.pdf}
         \label{tbl:imagenet-r-sample}
    \end{minipage} 
\end{table}




==> figs/05-analysis/objectnet-results.tex <==
\begin{table}[tpb]\footnotesize
    \begin{minipage}{.5\linewidth}
      \centering
 \setlength{\tabcolsep}{5pt}
               \captionsetup{width=.75\textwidth}
        \caption{GN and Fixup achieve the best results on ObjectNet.}
\tablefont
\begin{tabular}{lcc}
\multicolumn{3}{c}{ObjectNet evaluation (n = 512), accucary}\\
\toprule
ResNet50 model & top-1 & top-5 \\
\midrule
BatchNorm w/o adapt & 78.15 & 60.91 \\
BatchNorm w/ adapt & 75.96 & 58.85 \\
GroupNorm & \textbf{70.82} & \textbf{49.76} \\
Fixup &  71.48 & 51.44  \\
\bottomrule
\end{tabular}
      \label{tbl:objectnet}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
      
           \setlength{\tabcolsep}{5pt}
    \captionsetup{width=.75\textwidth}
    \caption{After shuffling IN-C corruptions, BN adaptation does not decrease the error.}

\tablefont
\begin{tabular}{lcc}
\multicolumn{3}{c}{Mixed IN-C, error}\\
\toprule
ResNet50 model & top-1 & top-5 \\
\midrule
BatchNorm w/o adapt & 61.08 &  40.81 \\
BatchNorm w/ adapt & 60.87 &  40.31 \\
GroupNorm & 57.25 &  35.97 \\
Fixup & \textbf{56.83} &  \textbf{35.43} \\
\bottomrule
\end{tabular}
      \label{tbl:mixed-inc}
    \end{minipage} 
\end{table}
